Diversity By Design: Leveraging Distribution Matching for Offline Model-Based Optimization

The goal of offline model-based optimization (MBO) is to propose new designs that maximize a reward function given only an offline dataset. However, an important desiderata is to also propose a diverse set of final candidates that capture many optimal and near-optimal design configurations. We propose Diversity in Adversarial Model-based Optimization (DynAMO) as a novel method to introduce design diversity as an explicit objective into any MBO problem. Our key insight is to formulate diversity as a distribution matching problem where the distribution of generated designs captures the inherent diversity contained within the offline dataset. Extensive experiments spanning multiple scientific domains show that DynAMO can be used with common optimization methods to significantly improve the diversity of proposed designs while still discovering high-quality candidates.

==> tables/story-qualitative.tex <==
\begin{table}[t]
\caption{Example top 4 designs for the \textbf{StoryGen} task generated using BO-qUCB optimizing against the baseline and DAAG-modified MBO objectives in a single representative experimental run. \textbf{\textit{FRES}}: Oracle Flesch Reading Ease Score \citep{flesch}.}
\label{story-qualitative}
%\vskip 0.15in
\begin{center}
\begin{small}
\centering
\begin{tabular}{p{6cm} c}
\toprule
\textbf{BO-qUCB Baseline MBO} & \textbf{FRES} $\uparrow$ \\
\midrule
To the Rams' inputs, they pointed to them. They pointed to zoom zoom zoom... & 100.4 \\
64-48ptptptepteometer needed on the line. 00 minutes... & 102.1 \\
Rageageage vandalism dude's peepder as needed for you to get her... & 80.2 \\
86 girl girl girl the girl girl maneaganaganza, 101xaganagan... & 88.3 \\
\bottomrule
\toprule
\textbf{BO-qUCB DAAG MBO} & \textbf{FRES} $\uparrow$ \\
\midrule
She had made that part of that way. She had only made that more he did... & 95.5 \\
Sheenaena Warsed out with their kids' attention!!! All of Your... & 94.2 \\
She allowed them to paint her work in pinked. They saw the boys who wore... & 78.6 \\
Socks and animals. They had to use them to restrain its own parts. Its... & 74.2 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}
